Faster Subset Selection for Matrices and Applications

We study subset selection for matrices defined as follows: given a matrix $\matX \in \R^{n \times m}$ ($m > n$) and an oversampling parameter $k$ ($n \le k \le m$), select a subset of $k$ columns from $\matX$ such that the pseudo-inverse of the subsampled matrix has as smallest norm as possible. In this work, we focus on the Frobenius and the spectral matrix norms. We describe several novel (deterministic and randomized) approximation algorithms for this problem with approximation bounds that are optimal up to constant factors. Additionally, we show that the combinatorial problem of finding a low-stretch spanning tree in an undirected graph corresponds to subset selection, and discuss various implications of this reduction.

==> HC_Applications_other.tex <==
\section{Other Applications}\label{sec:other}
\subsection{Column-Based Low-Rank Matrix Reconstruction}
\label{application:lowrank}
Suppose we want to build a low rank approximation of $\matA \in \R^{d \times m}$. For a rank parameter
$r$, let $\matA_r$ denote the best rank $r$ approximation to $\matA$. That is, $\matA_r$ minimizes $\TNorm{\matA-\matB}$,
where $\matB$ ranges on all rank $r$ matrices. It is well known that $\matA_r$
can be computed via the SVD. However,
SVD uses all the columns of $\matA$ to compute $\matA_r$. In some applications it is desirable to
to use only a small set of columns to build the low rank approximation. Let ${\cal S} \subseteq [m]$
be a set of columns. Define $\Pi_{{\cal S},r}(\matA) \in \R^{d \times m}$ to be the best rank $r$ approximation of $\matA$
within the columns space of $\matA_{\cal S}$, with respect to the spectral norm. The so-called column reconstruction problem is:
given an oversampling parameter $k \geq r$, find a subset ${\cal S}$ of cardinality at most $k$ such that
$\TNorm{\matA - \Pi_{{\cal S},r}(\matA)}$ is minimized. This problem has gathered considerable interest lately; see~\cite{BDM11a} and references therein.

It is natural to evaluate $\Pi_{{\cal S},r}(\matA)$ in terms of $\matA_r$. That is, provide approximation
bounds of the form $\TNorm{\matA - \Pi_{{\cal S},r}(\matA)} \le \alpha \cdot \TNorm{\matA - \matA_r}$.
Currently, the best deterministic algorithms appear in~\cite{BDM11a}. These algorithms
achieve asymptotically optimal upper bounds, but there is still room for improvement in terms of running time.

%Currently, the deterministic algorithm that achieves the best $\alpha$ is described in Theorem 12 of~\cite{BDM11a}. For a fixed $\matA$, $r < \rank(\matA)$, and $k > n$, the algorithm
%finds a subset ${\cal S}$ of $k$ columns such that
%$$\TNorm{\matA - \Pi_{{\cal S},r}(\matA)}\le \sqrt{2} \left(1 + \frac{1 + \sqrt{ (\rho-r)/k }}{ 1 - \sqrt{ r/k }}  \right) \cdot \TNorm{\matA - \matA_r\,.$$
%Notice that this bound is asymptotically $O(\rho/k)$. Theorem 17 in~\cite{BDM11a} establishes that this is asymptomatically optimal. The running time of the algorithm is
%$T_{SVD} + O\left(k m (r^2+\left(\rho-r\right)^2) \right)$ where $T_{SVD}$ is the time needed to compute all
%$\rho$ right singular vectors of $\matA$.

The algorithm of Corollary~\ref{cor1} can be used to obtain a new deterministic algorithm for the column reconstruction problem. First, construct an SVD decomposition $\matA = \matU \Sigma \matV\transp$. Let $\matY$ be the first $r$ rows of $\matV\transp$. We now use the algorithm of Corollary~\ref{cor1} on $\matY$ to generate a subset ${\cal S} \subseteq [m]$ of size $k$, which is the result of the algorithm. The following bound holds,
$$ \TNorm{\matA - \Pi_{{\cal S},r}(\matA)} \le \sqrt{2 + \frac{ r(m-k) }{ k - r + 1 }  }  \cdot \TNorm{\matA - \matA_r}\,.$$
We omit the proof, which follows by combining Lemma 7 from~\cite{Bou11a} and Corollary~\ref{cor1}. The algorithm is deterministic and the running time is $T_{SVD} + O(mr(m-k))$, where $T_{SVD}$ is the time needed to compute the top $r$ right singular vectors of $\matA$.
Our approximation bound is slightly worse than the bounds in~~\cite{BDM11a} but our running time can sometimes be better, depending on the size of the input matrix. We refer the interested reader to~\cite{BDM11a} to conduct her own comparison.
%
%For certain input matrices our algorithm is better than existing algorithms in terms of either running time or in terms of approximation bounds (possibly only up to constants), but worse in the other metric, For other matrices our algorithm is worse both in terms running time and in terms of approximation bound. In order to streamline the paper, we avoid laying out and analyzing all possible situations. We refer an interested reader to~\cite{BDM11a}, where he can learn the details of existing state-of-the-art algorithms and conduct his own comparison.

%We now compare the approximation bounds of the three algorithms described above. Assume that $\matA$ is a square full rank matrix of dimension $m$;
%let,
%$
%\alpha_1 = \sqrt{2} \left(2 + (\sqrt{ n(m-k) } ) (\sqrt{k - n + 1 }  ) \right);
%\alpha_2 = \sqrt{2} \left(1 + (1 + \sqrt{ (m-n)/k }) ( 1 - \sqrt{ n/k } )  \right);
%\alpha_3 = \sqrt{2} \left(1 + (1 + \sqrt{ m/k } ) (1 - \sqrt{ n/m }   ) \right).
%$
%For small $k$, say $k = \Theta(n)$: $\alpha_1 = O(m-n)$, $\alpha_2 = O(m/n)$, and $\alpha_3 = O(m/n)$.
%So, for reasonably large values of $m$ and $n$, the approximation bound of our algorithm is worse than
%existing bounds. Fortunately, for large $k$, say $k \rightarrow n$, our algorithm is not only faster than
%previous methods but also gives a better approximation bound by a small constant. Consider, for example,
%that $k=m-c$, where $c \le n$. Then, for any $n$, as $m \rightarrow \infty$, we obtain (via numerical tests),
%$
%\alpha_1 \rightarrow 2.82;
%\alpha_2  \rightarrow  4.24;
%\alpha_3  \rightarrow 4.24.
%$
%Notice that the ratios are $\alpha_2/\alpha_1 = \alpha_3/\alpha_1 \rightarrow 3/2$.
%In fact, these ratios hold for any $k \ge m - m^{\frac{946}{1000}}$, i.e $c \le m^{\frac{946}{1000}}$,
%provided that $m$ is sufficiently large.
%For $c \ge m^{\frac{947}{1000}}$, the ratios are smaller than $3/2$, and start getting closer to one until eventually becoming smaller than one.


%We now describe a novel deterministic algorithm to construct such a $\tilde\matA_n$. This algorithm
%runs in time $O\left( d m \min\{ d ,m\} + mn(m-k) +d m k + (d+m)k^2 \right)$ and guarantees that,
%$$ \TNorm{\matA - \tilde\matA_n} \le \sqrt{2} \left(2 + \sqrt{\frac{ n(m-k) }{ k - n + 1 }  }  \right) \cdot \TNorm{\matA - \matA_n}.$$
%(We commit the proof which follows by combining Lemma 7 of~\cite{BDM11a}, the spectral norm bound of
%Lemma 16 of~\cite{BDM11a}, and the spectral norm bound of our Corollary~\ref{cor1}). Given, $\matA$, $n$, and $k\ge n$,
%the algorithm is as follows:
%(i) apply Corollary~\ref{cor1} on the first $n$ rows of the matrix $\matV\transp$ from the SVD of $\matA$, $\matA = \matU \Sigma \matV\transp$;
%(ii) let, $\matC = \matA_{\cal S}$ and
%compute a $QR$ factorization $\matC = \matQ \matR$ with $\matQ \in \R^{d \times k}$ and $\matR \in \R^{k \times k}$;
%(iii) return $\tilde\matA_n = \matQ (\matQ\transp \matA)_n \in \R^{d \times m},$ where
%$ \left(\matQ\transp \matA \right)_n = \arg \min_{\matZ \in \R^{k \times m}, \rank(\matZ)\le n} \TNorm{\matQ\transp \matA - \matZ }.$
%
%Our algorithm improves upon the running time of the algorithm of~\cite{BDM11a}. To see this, notice
%that the term $mn(m-k)$ is always better than $km\left(n^2+\left(\rho-n\right)^2\right)$. For large $k$, this improvement can be a lot. We should mention though that~\cite{BDM11a} provides another deterministic algorithm (see Theorem 12 in~\cite{BDM11a}), which, for $k > n$,
%achieves almost the same bound in $O\left( d m \min\{ d,m\} + mn^2k + dmk + (d+m)k^2 \right)$ time:
%$ \TNorm{\matA - \tilde\matA_n} \le \sqrt{2} \left(1 + (1 + \sqrt{ m/k }) /( 1 - \sqrt{ n/k } )  \right) \cdot \TNorm{\matA - \matA_n}.$
%In this case, one should compare the term $ mn(m-k)$ of our algorithm with the term $mn^2k$ in the method of~\cite{BDM11a}. Our algorithm is faster only if $m-k = o(nk)$; for example, our method is particularly appealing if  $k \rightarrow m$.


\subsection{Sparse Solutions to Least-squares Regression Problems}\label{application:sparse}
Fix inputs $\matA \in \R^{d \times m}$ and $\b \in \R^d$; consider the following least-squares problem,
$ \min_{\x \in \R^m} \TNorm{\matA \x - \b}$.
Since there is no assumption on $d$ and $m$, or that $\matA$ is full rank, the minimizer of $\TNorm{\matA \x - \b}$
might not be unique; there might be a full subspace of minimizers. Even if there is a unique minimizer, it might have
a huge norm, while there exists an almost-minimizer with small norm. It depends on the application
what exactly is needed, but often some kind of \emph{regularization} is used to address the issues just mentioned.
One popular regularization technique is \emph{truncated SVD}~\cite{Han87}: for $r < \rank(\matA)$,
let $\matA_r \in \R^{d \times m}$ of rank $r$ denotes
the rank-$r$ SVD of $\matA$; then, the truncated SVD regularized
solution is given by
$
\x_{svd(r)}=\matA_r^{+}\b \in \R^{m}
$.

However, sometimes a different regularization is sought: requiring the solution vector to be sparse.
That is, we are interested in constructing a vector $\x_k \in \R^m$ that has at most $k$ non-zeros, for some
$k$. Since truncated SVD is arguably the most natural
regularizer, it makes sense to compare $\x_k$ to $\x_{svd(r)}$ for some $r \leq k$. More specifically, we are interested in bounds of the form,
$$ \TNorm{\matA \x_k - \b} \le \TNorm{\matA \x_{svd(r)} - \b} + \alpha\,.$$
The idea of obtaining sparse solutions
with approximation bounds of the above type can be traced to~\cite{CH92}. Currently, the best \emph{deterministic}
method is in~\cite{Bou11b} ($k>r$) with $\alpha = \left(1+\sqrt{\frac{r}{k}} \right) \norm{\b}_2 \FNorm{\matA-\matA_r} / \sigma_{r}(\matA)$.

The algorithm of Corollary~\ref{cor1} can be used to obtain a new deterministic algorithm. First, construct an SVD decomposition $\matA = \matU \Sigma \matV\transp$. Let $\matY$ be the first $r$ rows of $\matV\transp$. We now use the algorithm of Corollary~\ref{cor1} on $\matY$ to generate a subset ${\cal S} \subseteq [m]$ of size $k$.  We now compute $\hat{\x}_k = \matA^+_{\cal S} \b \in \R^k$. We form $\x_k$ by spreading the indices of $\hat{\x}_k$ to their corresponding place in $\x_k$ and putting $0$ elsewhere. The following bound holds,
$$
\TNorm{\matA \x_k-\b}
\le
\TNorm{ \matA \x_{svd(r)}-\b} + \left(1+\sqrt{\frac{r(m-k)}{k-r+1}} \right) \norm{\b}_2 \frac{\sigma_{r+1}(\matA)}{\sigma_{r}(\matA)}\,.
$$
We omit the proof since it follows immediately by combining Lemma 3 from~\cite{Bou11b} with
Corollary~\ref{cor1}. The algorithm is deterministic and the running time is $O(d m \min\{d,m\} + mr(m-k))$.

Our bound essentially contains the term $\sqrt{m-k} \cdot \sigma_{r+1}(\matA)$ in place of the term $\FNorm{\matA-\matA_r}$ in the bound of~\cite{Bou11b}. It is always the case that $\FNorm{\matA-\matA_r} \le \sqrt{m-r} \cdot \sigma_{r+1}(\matA)$, but since $k \ge r$, our bound might be better in some cases (e.g. when $k \rightarrow m$).



\subsection{Feature Selection in $k$-Means Clustering}\label{application:kmeans}
The deterministic algorithm of Corollary~\ref{cor1} can also be
used for deterministic feature selection in $k$-means clustering. We refer
the reader to~\cite{BM11} for an introduction to this problem. Theorem 4 of~\cite{BM11}
gives such a poly-time deterministic unsupervised feature selection algorithm, which selects features from the data and then \emph{rescales} them.
Using Corollary~\ref{cor1}, one can design a deterministic unsupervised feature selection algorithm \emph{without} rescaling.
We omit the details, since the algorithm is similar to the one described for sparse least squares, and
the analysis is  a combination of Lemma 10 from~\cite{BM11} with Corollary~\ref{cor1}. The approximation bound
that is obtained is $O( r(m-k) / (k-r+1))$; here,
$m$ is the number of features in the input points, $r$ is the number of clusters, and $k$ is the number of features after feature selection.


%Consider $d$ points in an $m$-dimensional Eucledian space,
%$\mathcal{P} = \{ \z_1, \z_2, ..., \z_d \} \in \R^m,$ and integer
%$n$ denoting the number of clusters. The objective of
%Kmeans clustering is to find an $n$-partition of
%$\mathcal{P}$ such that points that are ``close'' to each other belong to the same cluster and points
%that are ``far'' from each other belong to different clusters.
%A $n$-partition of $\mathcal{P}$ is a collection
%$\cl S=\{\mathcal{S}_1, \mathcal{S}_2, ..., \mathcal{S}_n\}$
%of \math{n} non-empty pairwise disjoint
%sets which covers \math{\cl P}.
%Let $s_j=|\mathcal{S}_j|,$ be the size of $\mathcal{S}_j$.
%Let
%$\matA\transp=[\z_1, \z_2,\ldots,\z_d].$ has dimensions $m \times d$.
%We represent a clustering \math{\cl S} by its cluster indicator matrix
%$\matX \in \R^{d \times n}$.
%Each column \math{j=1,\ldots,n} of \math{\matX} represents a cluster.
%Each row \math{i=1,\ldots,d}
%indicates the
%cluster membership of the point \math{\z_i}. So,
%$\matX_{ij}=1/\sqrt{s_j},$ if and
%only if data point \math{\z_i} is in cluster \math{S_j} ($s_j = |\cl S_j|$).
%Every row of $\matX$ has one non-zero element,
%corresponding to the cluster the data
%point belongs to. There are \math{s_j} non-zero elements in column
%\math{j}, which indicates the points belonging to
%\math{S_j}.
%The goal of Kmeans is to find an indicator
%matrix $\matX$ which minimizes \math{\FNormS{\matA - \matX \matX\transp \matA}}.
%We will denote the best such matrix with,
%$ \matX_{opt} = \arg \min_{\matX \in \R^{d \times n}} \FNormS{ \matA - \matX \matX\transp \matA };$
%so,
%$\cl F_{opt} = \FNormS{\matA - \matX_{opt} \matX_{opt}\transp \matA}.$
%The goal of feature selection is to construct points $\matC \in \R^{d \times k}$, where $\matC$
%is a subset of $k$ columns from $\matA$.
%Now consider the optimum Kmeans partition of the points in $\matC$,
%$ \hat{\matX}_{opt} = \arg \min_{\matX \in \R^{d \times n}} \FNormS{ \matC - \matX \matX\transp \matC }.$
%The goal of feature selection is to construct  $\matC$ such that,
%$$ \FNormS{ \matA - \hat{\matX}_{opt} \hat{\matX}_{opt}\transp \matA } \leq \alpha \cdot \FNormS{ \matA - \matX_{opt} \matX_{opt}\transp \matA }.$$
%Here, $\alpha$ is the approximation which depends on $d,m,n$ and $k$.
%Feature selection has been studied extensively in the literature both empirically~\cite{GE03,GGBD05,HCN06,ZCZ08} and
%theoretically~\cite{BMD09b,BZMD11,BM11}. The former approach provides algorithms that do not offer an upper bound for $\alpha$. The later
%gives algorithms with approximation guarantees. The best such \emph{deterministic} algorithm (see ~\cite{BMD09b,BZMD11} for better randomized algorithms)
%is in~\cite{BM11} (specifically Theorem 4) and
%describes an unsupervised feature selection $O(d m \min\{d,m\} + kn^2m)$ time algorithm which, on input the dataset
%$\matA \in \R^{d \times m}$, the number of clusters $n$, and the number of features $k > n$, constructs $\matC \in \R^{d \times k}$ with $k$
%rescaled columns of $\matA$ such that,
%$$ \FNormS{ \matA - \hat{\matX}_{opt} \hat{\matX}_{opt}\transp \matA } \leq
%\left(1 + 4 \left( 1 + \sqrt{m/k}\right)^2 \left(1 - \sqrt{n/k} \right)^{-2}  \right) \cdot \FNormS{ \matA - \matX_{opt} \matX_{opt}\transp \matA }.$$
%For large enough $k$, the approximation bound is of the order $O(m/k)$. Via using the algorithm of Corollary~\ref{cor1}, we will now
%describe a novel unsupervised feature selection deterministic algorithm.
%\begin{theorem}
%Fix $\matA \in \R^{d \times m}$, number of clusters $n$, and number of features $k \ge n$.
%There is an $O(d m \min\{d,m\} + mn(m-k))$ time deterministic algorithm which constructs $\matC$ with $k$ columns of $\matA$, such that
%$$ \FNormS{ \matA - \hat{\matX}_{opt} \hat{\matX}_{opt}\transp \matA } \leq
%\left(1 + 4 \left( 1 + \frac{n(m-k)}{k-n+1} \right) \right) \cdot \FNormS{ \matA - \matX_{opt} \matX_{opt}\transp \matA }.$$
%\end{theorem}
%\begin{proof}
%The algorithm consists of applying the algorithm of Corollary~\ref{cor1} to the matrix $\matV_n\transp \in \R^{n \times m}$ of the top $n$
%right singular vectors of $\matA$ and, then, selecting the corresponding columns in $\matA$. To prove our bound, it suffices
%to combine Lemma 10 from~\cite{BM11} with Corollary~\ref{cor1}. Lemma 10 from~\cite{BM11} indicates that,
%for any sampling matrix $\matS$, if $\rank(\matV_n\transp \matS) = n$:
%$
% \FNormS{ \matA - \hat{\matX}_{opt} \hat{\matX}_{opt}\transp \matA } \leq
%\left(1 +
%4  \cdot \TNormS{(\matV_n\transp\matS)^+} \right) \cdot \FNormS{(\matA -\matX_{opt} \matX_{opt}\transp \matA) \matS}.
%$
%Using our bounds for $\TNormS{(\matV_n\transp)^+}$ concludes the proof.
%\end{proof}
%
%\subsubsection*{Discussion}
%Notice that we were able to achieve almost the same bound as the one in Theorem 4 of~\cite{BM11} \emph{without} rescaling the features.
%The comparison of the running times and approximation bounds of our algorithm and the one in~\cite{BM11}
%is similar to the one we provided in section~\ref{application:lowrank}. We should highlight though that the
%new method is particularly appealing if one wants to \emph{remove}  a small number of features in Kmeans clustering.


==> HC_GreedySelection.tex <==
\section{Two-stage Deterministic Greedy Selection}
Next, we describe a deterministic algorithm which selects columns from $\matX$ in two different stages.
In the first stage, we select $n$ columns from $\matX$ via the Strong RRQR algorithm from~\cite{GE96};
then, in the second stage, we select another $k-n$ columns with a greedy procedure similar to Theorem 1,
which, in turn, is similar to Theorem 2 in~\cite{HM07}. However, in our theorem below we start with the
$n$ columns found in the first stage and, then, we add columns by \emph{selecting} one column from the
remaining columns of $\matX$ at a time. The algorithm in Theorem 1 starts with $\matX$
and proceeds by \emph{removing} columns one at a time. Because of this feature, our algorithm here is
considerably faster when $k$ is small.

\begin{theorem}\label{thm5}
Fix $\matX \in \R^{n \times m}$ ($m\ge$, $\rank(\matX)=n$) and oversampling parameter $k \ge n$.
There is an $O\left( mn^2 \log m + mnk \right)$ time
deterministic algorithm which constructs a set $\cal S$ $\subseteq [m]$ of cardinality $k$ such that,
$$
\FNormS{  \matX_{ \cal S}^+ } \le  \frac{ 4(m-n) + 1}{\left(k-n\right) \left( 1 + \frac{n-1}{m-n+1}\right) } \cdot n \cdot \TNormS{\matX^+}.
$$
Also,
for $i=1,\dots,n$,
$$\sigma^{-2}_i\left(\matX_{\cal S}\right) \leq \left(1+\frac{n \left(4m-3n-k+1\right)}{\left(k-n\right) \left( 1 + \frac{n-1}{m-n-1}\right)} \right) \cdot \sigma^{-2}_i\left(\matX\right)\,.$$
In particular,
$$\TNormS{\matX_{\cal S}^{+}} \leq \left(1+\frac{n \left(4m-3n-k+1 \right)}{\left(k-n\right) \left( 1 + \frac{n}{m-n-1}\right)} \right) \cdot \TNormS{\matX^{+}}\,.$$
\end{theorem}
\begin{proof}
We first state the algorithm; then, we prove the approximation bounds. Finally, we analyze the running time.

\paragraph{Algorithm.}
First, we compute the SVD of $\matX$: $\matX = \matU \Sigma\matV\transp$. Let,
$\matV\transp = \matY = [\y_1, \y_2,...,\y_m] \in \R^{n \times m},$
be the column representation of $\matY$, with $\y_i$'s $\in \R^n$.
In fact, we only need the right singular vectors of $\matX$.
We now describe a two-stage procedure which selects $k$ column indices
from $\matY$; we return the corresponding indices (columns) in $\matX$.

In the first stage of this procedure, we run Algorithm 4 of~\cite{GE96} ($f=2$) with inputs a rank parameter $n$ and an $m \times m$ matrix $\matA$,
whose first $n$ rows are $\matY$ and whose other rows are all-zeros,
$$ \matA =  \left( \begin{array}{cc} \matY            \\
                {\bf 0}_{(m-n) \times m}  \end{array} \right) \in \R^{m \times m}.$$
The output of Algorithm 4 of~\cite{GE96} on inputs $\matA$ and rank parameter $n$ is a permutation matrix $\Pi \in \R^{m \times m}$,
$$ \matA \Pi =  \left( \begin{array}{cc} \matY_{{\cal S}_n}           & \matY_{\bar{{\cal S}}_n} \\
                                         {\bf 0}_{(m-n) \times n} & {\bf 0}_{(m-n) \times (m-n)}  \end{array} \right).$$
Here, ${\cal S}_n$ is a subset of cardinality $n$ and $\bar{{\cal S}}_n = [m] - {\cal S}_n$, has cardinality $m-n$.
Without loss of generality, and for simplicity in our presentation, we assume that ${\cal S}_n = \{1,2,...,n\}$, i.e. $\Pi = \matI_m$; so,
$$ \matY_{\bar{{\cal S}}_n} = [\y_{n+1}, \y_{n+2},...,\y_m] \in \R^{n \times (m-n)}.$$
In the second stage of this procedure, which, in turn, proceeds in $k-n$ iterations, we select another $k-n$ columns of $\matY_{\bar{{\cal S}}_n}$ as follows.
In the first iteration, we select the column with index $i_1$ such that,
$$ i_1 = \arg \min_{i=n+1,n+2,...,m} \trace\left(  \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n} \transp + \y_i \y_i\transp \right)^{-1}  \right). $$
Let $\matY_1 \in \R^{n \times (n+1)}$ be the matrix after inserting to $\matY_{{\cal S}_n} \in \R^{n \times n}$ the $i_1$th column of $\matY$ just selected above,
$$ \matY_1 =  \left( \begin{array}{cc} \matY_{{\cal S}_n} & \y_{i_1}   \end{array} \right) \in \R^{n \times (n+1)}.$$
Without loss of generality, and for simplicity in our presentation, let $\y_{i_1} = \y_{n+1}$.
In the second iteration, we select the column with index $i_2$ such that,
$$ i_2 = \arg \min_{i=n+2,n+3,...,m} \trace\left(  \left( \matY_1 \matY_1\transp + \y_i \y_i\transp \right)^{-1}  \right), $$
and so on, until $k-n$ columns are selected. Finally, we return ${\cal S} = {\cal S}_n + \{i_1, i_2,...,i_{k-n}\}$, which contains $k$ indices.

\paragraph{Approximation bound (Frobenius norm).} %We first prove the Frobenius norm bound in the theorem.
Notice that, if $\rank(\matY_{\cal S}) = n$, then,
$$\FNormS{ \matX_{\cal S}^+ } =
  \FNormS{ \left(\matU \Sigma \matY_{\cal S}\right)^+ } =
  \FNormS{\matY_{\cal S}^+ \left(\matU \Sigma\right)^+  } \le
  \FNormS{ \matY_{\cal S}^+ } \cdot \TNormS{ \left(\matU \Sigma\right)^+}  =
  \FNormS{\matY_{\cal S}^+} \cdot \TNormS{\matX^+}.$$
Below, we show that the set ${\cal S} \subseteq [m]$ of our algorithm satisfies the rank assumption and the following upper bound,
$$ \FNormS{\matY_{\cal S}^+} \le \frac{ 4(m-n) + 1}{\left(k-n\right) \left( 1 + \frac{n-1}{m-n-1}\right) } \cdot n.$$
Replacing this bound in $\FNormS{ \matX_{\cal S}^+ } \le  \FNormS{\matY_{\cal S}^+} \TNormS{\matX^+},$ gives the Frobenius norm bound in the theorem.

Recall that in the first stage of the algorithm we constructed a set ${\cal S}_n$ with $n$ indices:
$ \matY \Pi =  \left( \begin{array}{cc} \matY_{{\cal S}_n}  & \matY_{\bar{{\cal S}}_n}  \end{array} \right).$
We first show that $\matY_{{\cal S}_n}$ is a full rank matrix, which also implies that $\rank(\matY_{\cal S}) = n$.
Eqn.~(8) in Theorem 3.2 in~\cite{GE96},
which shows that $ \sigma_n( \matY_{{\cal S}_n} ) \ge \sigma_n(\matA) \left(1+4n(m-n) \right)^{-1}$,
along with the fact that $\sigma_n(\matA) = \sigma_n(\matY) = 1$, implies that $\sigma_n( \matY_{{\cal S}_n} ) > 0$,
which, in turn, implies that $\rank( \matY_{{\cal S}_n} ) = n$.
We now provide an upper bound for  $\FNormS{ \matY_{{\cal S}_n}^{-1} }$.
The proof of Theorem 3.2 in~\cite{GE96} with $f=2$ shows that $ \FNormS{ \matY_{{\cal S}_n}^{-1} \matY_{\bar{{\cal S}}_n} } \le 4 (m-n) n$.
This bound is implicitly proven in the calculations after eqn.~(10), and follows by the fact that, for $i=1:n$, $j=1:m-n$, the $(i,j)$th element
of $\matY_{{\cal S}_n}^{-1} \matY_{\bar{{\cal S}}_n}$ satisfies $ \left( \matY_{{\cal S}_n}^{-1} \matY_{\bar{{\cal S}}_n} \right)_{ij}^2 \le f^2$,
which, in turn, follows by the fact that $\left( \matY_{{\cal S}_n}^{-1} \matY_{\bar{{\cal S}}_n} \right)_{ij}^2 = \frac{\det(\matY_{\cal S}(i \rightarrow \y_{n+j}))}{\det(\matY_{\cal S})} \le f^2$. Now, eqn.~(4) in~\cite{HM07} indicates that
$ \FNormS{ \matY_{{\cal S}_n}^{-1} } \le \rank(\matY_{{\cal S}_n})  + \FNormS{ \matY_{{\cal S}_n}^{-1} \matY_{\bar{{\cal S}}_n} }$.
Combining this inequality with the upper bound for $\FNormS{ \matY_{{\cal S}_n}^{-1} \matY_{\bar{{\cal S}}_n} }$, we obtain,
$$ \FNormS{ \matY_{{\cal S}_n}^{-1} } \le  \left(4 \left( m-n \right) + 1 \right) n .$$



We now analyze the second stage of the algorithm. For $i=1,2,...,m,$ let us denote
$ \q_i = (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \y_i \in \R^n$. Notice
that $(\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \in \R^{n \times n}$ is well defined
because $\rank( \matY_{{\cal S}_n} ) = n$.
Notice also that since $\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp$ is full rank,
$\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp + \y_i \y_i\transp$ is full rank as well for any $i=n+1,...,m$.
So, we can calculate the inverse of
$\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp + \y_i \y_i\transp$ using the Sherman-Morisson formula.  For $i=n+1,n+2,...,m:$
$$  \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp + \y_i \y_i\transp \right)^{-1}  =
    \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} - \frac{
    \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} \y_i \y_i\transp \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1}}
    {1 + \y_i\transp \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} \y_i}.
$$
The way we selected the index $i_1$ implies that for $i=n+1,n+2,...,m:$
$$ \trace\left(  \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n} \transp + \y_{i_1} \y_{i_1}\transp \right)^{-1}  \right) \le
\trace\left(  \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n} \transp + \y_{i} \y_{i}\transp \right)^{-1}  \right) =
\trace\left( \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} -
\frac{
    \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} \y_i \y_i\transp \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1}}
    {1 + \y_i\transp \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} \y_i}
\right)
,$$
where the equality follows by the previous identity.
Now, for each $i=n+1,n+2,...,m$ multiply both sides of this inequality with $(1 + \TNormS{\q_i}) > 0$ and use the linearity of the trace operator,
$$ (1 + \TNormS{\q_i}) \cdot \trace\left(  \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n} \transp + \y_{i_1} \y_{i_1}\transp \right)^{-1}  \right)  \le
(1 + \TNormS{\q_i}) \cdot \trace\left( \left( \matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} \right) -
    \trace\left( \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1} \y_i \y_i\transp \left(\matY_{{\cal S}_n} \matY_{{\cal S}_n }\transp\right)^{-1}
\right)
.$$
Now, replace the traces with the Frobenius norm of appropriate matrices. So, again, for $i=n+1,...,m$ we obtain,
$$ (1 + \TNormS{\q_i}) \cdot \FNormS{  \matY_1^{+}  } \le
   (1 + \TNormS{\q_i}) \cdot \FNormS{   \matY_{{\cal S}_n}^{+}  }  -
                            \TNormS{ (\matY_{{\cal S}_n} \matY_{{\cal S}_n}\transp)^{-1} \y_i }.
$$
Summing these equations over $i=n+1,n+2,...,m$, we obtain,
$$ \FNormS{  \matY_1^{+}  } \cdot \sum_{i=n+1}^m (1 + \TNormS{\q_i})  \le \FNormS{   \matY_{{\cal S}_n}^{+}  } \cdot
\sum_{i=n+1}^m  (1 + \TNormS{\q_i}) \  -  \sum_{i=n+1}^m  \TNormS{ (\matY_{{\cal S}_n} \matY_{{\cal S}_n}\transp)^{-1} \y_i } .
$$
Replacing the summand,
$$ \sum_{i=n+1}^m  (1 + \TNormS{\q_i}) = m - n + \sum_{i=n+1}^m  \TNormS{\q_i},$$
and multiplying both sides of the inequality with $\left(m - n + \sum_{i=n+1}^m  \TNormS{\q_i}\right)^{-1} > 0$, we obtain,
$$ \FNormS{ \matY_1^+ } \le
\FNormS{\matY_{{\cal S}_n}^+ } - \frac{\sum_{i=n+1}^m \TNormS{(\matY_{{\cal S}_n} \matY_{{\cal S}_n}\transp)^{-1} \y_i }}{m-n+\sum_{i=n+1}^m \TNormS{\q_i}}.
$$
On noting that,
 \begin{eqnarray*}
\sum_{i=n+1}^m \TNormS{(\matY_{{\cal S}_n} \matY_{{\cal S}_n}\transp)^{-1} \y_i }
&=& \sum_{i=1}^m \TNormS{(\matY_{{\cal S}_n} \matY_{{\cal S}_n}\transp)^{-1} \y_i } - \sum_{i=1}^n \TNormS{(\matY_{{\cal S}_n} \matY_{{\cal S}_n}\transp)^{-1} \y_i } \\
&=& \sum_{i=1}^m \trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \y_i \y_i\transp (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right) -
\sum_{i=1}^n \trace\left( (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \y_i \y_i\transp (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right)\\
&=& \trace\left( \sum_{i=1}^m (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \y_i \y_i\transp (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right) -
\trace\left( \sum_{i=1}^n (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \y_i \y_i\transp (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right)\\
&=& \trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \left( \sum_{i=1}^m\y_i \y_i\transp \right) (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right) -
\trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \left(\sum_{i=1}^n\y_i \y_i\transp \right) (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right)\\
&=& \trace\left( (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \matI_n (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right) -
\trace\left( (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp ) (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right)\\
&=& \trace\left( (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-2}  \right) -\trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1} \right)\\
&=& \sum_{j=1}^n \frac{1}{ \sigma_j^4 \left( \matY_{ {\cal S}_n } \right)} - \sum_{j=1}^n \frac{1}{ \sigma_j^2 \left( \matY_{ {\cal S}_n } \right)} \\
&=& \sum_{j=1}^n \frac{1}{ \sigma_j^4 \left( \matY_{ {\cal S}_n } \right)} - \FNormS{ \matY_{{\cal S}_n}^+ }\\
\end{eqnarray*}
and,
\begin{eqnarray*}
\sum_{i=n+1}^m  \TNormS{\q_i} &=& \sum_{i=1}^m  \TNormS{\q_i} - \sum_{i=1}^n  \TNormS{\q_i} \\
&=& \sum_{i=1}^m \trace\left( \q_i \q_i\transp \right) - \sum_{i=1}^n\trace\left( \q_i \q_i\transp \right) \\
&=& \trace\left( \sum_{i=1}^m \q_i \q_i\transp \right) - \trace\left( \sum_{i=1}^n \q_i \q_i\transp \right) \\
&=&
\trace\left( \sum_{i=1}^m (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \y_i \y_i\transp (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \right) -
\trace\left( \sum_{i=1}^n (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \y_i \y_i\transp (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \right) \\
&=&
\trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \left(\sum_{i=1}^m \y_i \y_i\transp\right) (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \right) -
\trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \left(\sum_{i=1}^n \y_i \y_i\transp\right) (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \right) \\
&=&
\trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \matI_n (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \right)  -
\trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )
(\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-\frac{1}{2}} \right) \\
&=&
\trace\left(  (\matY_{{\cal S}_n} \matY_{ {\cal S}_n }\transp )^{-1}  \right)  -
\trace\left(  \matI_n \right) \\
&=&  \FNormS{ \matY_{{\cal S}_n}^+} - n,
\end{eqnarray*}
we obtain,
$$ \FNormS{ \matY_1^+ } \le
\FNormS{\matY_{{\cal S}_n}^+ } + \frac{\FNormS{\matY_{{\cal S}_n}^+ } - \sum_{j=1}^n  \sigma_j^{-4} \left( \matY_{ {\cal S}_n } \right)} {m-n+\FNormS{\matY_{{\cal S}_n}^+}-n}
$$
XXX up to here should be ok - commented out the rest of the proof XXX

Now, the interlacing property of the singular values indicates that for $j=1,...,n,$ $\sigma_j(\matY_{\cal S}) \le \sigma_j(\matY) = 1$. This
implies that $ - \sum_{j=1}^n  \sigma_j^{-4} \left( \matY_{ {\cal S}_n } \right) \le - n$ and  $ \FNormS{\matY_{{\cal S}_n}^+} \ge n$; so,
$$ \FNormS{ \matY_1^+ } \le
\FNormS{\matY_{{\cal S}_n}^+ } + \frac{\FNormS{\matY_{{\cal S}_n}^+ } - n} {m-n+n-n} =
\FNormS{\matY_{{\cal S}_n}^+ } + \frac{\FNormS{\matY_{{\cal S}_n}^+ } - n} {m-n} =
\frac{ (m-n+1) \FNormS{\matY_{{\cal S}_n}^+ } - n }{ m-n } \le
\frac{ \FNormS{\matY_{{\cal S}_n}^+}  }{1 - \frac{1}{(m-n+1)} } \le
\frac{ 4 (m-n) + 1 }{ 1 - \frac{ 1 }{m-n+1} } \cdot n.
$$
In the above, the second inequality follows by first dropping the term $n$ from the enumerator, then, adding $+1-1$ in the enumerator, and, finally, multiplying both the numerator and the denominator with $(m-n +1)^{-1}> 0$. The last inequality follows by the upper bound of $\FNormS{\matY_{{\cal S}_n}^+ }$. In summary so far, we obtain,
$$ \FNormS{ \matY_1^+ } \le \frac{ 4 (m-n) + 1 }{ 1 - \frac{ 1 }{m-n+1} } \cdot n,$$
which is a bound for $\FNormS{ \matY_1^+ }$ but this only corresponds to $k=n+1$, i.e. one step of the second stage of our algorithm.
Next, we outline how one can obtain similar bounds for $\FNormS{ \matY_2^+ }, \FNormS{ \matY_3^+ },...,\FNormS{ \matY_{k-n}^+ }$.
Note that $ \matY_{k-n} = \matY_{\cal S}$, so we eventually get a bound for the term $\FNormS{ \matY_{\cal S}^+ }$, which is all we need to conclude the proof.
XXX up to here should be fine XXX
Let $\matY_2 \in \R^{n \times (n+2)}$ be the matrix after appending to $\matY_1$ the column of $\matY$ with index $i_2$. Then
\begin{eqnarray*}
 \FNormS{ \matY_1^+ }
 \le   \FNormS{\matY_{{\cal S}_n}^+ } - \frac{\sum_{i=n+1}^m \TNormS{(\matY_{{\cal S}_n} \matY_{{\cal S}_n}\transp)^{-1} \y_i }}{m-n+\sum_{i=n+1}^m \TNormS{\q_i}}
 &\le& \FNormS{\matY_{{\cal S}_n}^+ } + \frac{\FNormS{\matY_{{\cal S}_n}^+ } - n} {m-n+n-n} \\
 &=&   \FNormS{\matY_{{\cal S}_n}^+ } + \frac{\FNormS{\matY_{{\cal S}_n}^+ } - n} {m-n} \\
 &=&   \frac{ (m-n+1) \FNormS{\matY_{{\cal S}_n}^+ } - n }{ m-n } \\
 &\le& \frac{ \FNormS{\matY_{{\cal S}_n}^+}  }{1 - \frac{1}{(m-n+1)} } \\
 &\le& \frac{ 4 (m-n) + 1 }{ 1 - \frac{ 1 }{m-n+1} } \cdot n.
\end{eqnarray*}


$$ \FNormS{ \matY_2^+ } \le
\frac{ ( (m-n-1)+1) \cdot \FNormS{\matY_1^+ }  }{(m-n-1)+\FNormS{\matY_1^+ }} \le
\frac{ ((m-n-1)+1) \cdot \FNormS{\matY_1^+ }  }{(m-n-1) + n} =
\frac{ ((m-n-1)+1) \cdot \FNormS{\matY_1^+ }  }{(m-n-1+1) + (n - 1)} =
\frac{  \FNormS{\matY_1^+ }  }{1+ \frac{n-1}{m-n-1+1}}.$$
So, using the upper bound for $\FNormS{\matY_1^+ }$ we can derive an upper bound for $\FNormS{\matY_2^+ }$ as follows,
$$
\FNormS{ \matY_2^+ } \le \frac{ 4 (m-n) + 1 }{ \left(1 + \frac{n-1}{m-n+1} \right) \left(1 + \frac{n-1}{m-n} \right) } \cdot n,
$$
In fact, for any $j=2,3,...,k-n$ the following bound holds ($\FNormS{\matY_j^+ } \ge n$),
\begin{eqnarray*}
\FNormS{ \matY_j^+ } \le
\frac{ ( (m-n-(j-1))+1) \cdot \FNormS{\matY_{j-1}^+ }  }{(m-n-(j-1))+\FNormS{\matY_{j-1}^+ }}  &\le&
\frac{ ((m-n-(j-1))+1) \cdot \FNormS{\matY_{j-1}^+ }  }{(m-n-(j-1)) + n} \\ &=&
\frac{ ((m-n-(j-1))+1) \cdot \FNormS{\matY_{j-1}^+ }  }{(m-n-(j-1)+1) + (n - 1)} \\ &=&
\frac{  \FNormS{\matY_{j-1}^+ }  }{1+ \frac{n-1}{m-n-(j-1)+1}}.
\end{eqnarray*}
So, for any $j=2,3,...,k-n$, using the upper bound for $\FNormS{\matY_{j-1}^+ }$ we can derive an upper bound for $\FNormS{\matY_j^+ }$,
$$
\FNormS{ \matY_j^+ } \le \frac{  \FNormS{\matY_{j-1}^+ }  }{1+ \frac{n-1}{m-n-j+2}}.
$$
We conclude the proof by using the bounds inductively for $j=k-n, k-n-1,...,1$, and the fact that $k \ge n + 1 $,
\begin{eqnarray*}
\FNormS{ \matY_{\cal S}^+ }  = \FNormS{ \matY_{k-n}^+ } &\le&
\frac{ 4(m-n)+1 }{ \left(1 + \frac{n-1}{m-n+1} \right) \left(1 + \frac{n-1}{m-n} \right) \dots \left(1 + \frac{n-1}{m-k+2} \right)} \cdot n \\
&\le&
\frac{ 4(m-n)+1 }{ \underbrace{\left(1 + \frac{n-1}{m-n+1} \right) \left(1 + \frac{n-1}{m-n+1} \right) \dots \left(1 + \frac{n-1}{m-n+1} \right)}_{(k-n)-times}} \cdot n \\
&=&
\frac{ 4(m-n)+1 }{ \left( k-n \right) \left(1 + \frac{n-1}{m-n+1} \right)} \cdot n.
\end{eqnarray*}

\paragraph{Approximation bound (singular values).}
We now prove the bounds for the singular values of $\matX_{\cal S}$.
Let,
$$
\matW = \left(\begin{array}{cc}
             \matI_k & \matX_{\cal S}^{+}\matX_{\bar{\cal S}} \\
             {\bf 0}_{(m-k) \times k} & \matI_{m-k}
          \end{array}
    \right)\in \R^{m \times m}\,.
$$
(Note that $\matX_{\cal S}^{+}\matX_{\bar{\cal S}}\in \R^{k \times (m-k)}$). Since $\matX_{\cal S}$ has full rank, we have
$$\left( \begin{array}{cc} \matX_{\cal S} & {\bf 0}_{n \times (m-k)} \end{array} \right) \matW =
\left( \begin{array}{cc} \matX_{\cal S} & \matX_{\bar{\cal S}} \end{array} \right) = \matX \Pi.
$$
Clearly $\matW$ is non-singular (it is a triangular matrix with a non-zero diagonal), so for $i=1,\dots,n$,
$$
\sigma^{-2}_i \left( \matX_{\cal S} \right) =
    \sigma^{-2}_i \left( \left( \begin{array}{cc} \matX_{\cal S} & {\bf 0}_{n \times (m-k)} \end{array} \right) \right ) =
    \sigma^{-2}_i \left( \matX \Pi \matW^{-1} \right) \leq
    \TNormS{\matW} \cdot \sigma^{-2}_i \left( \matX \right) \,.
$$
To bound $\TNormS{\matW}$ we observe that,
$$\TNormS{\matW} \le 1 + \TNormS{\matX_{\cal S}^+ \matX_{\bar{\cal S}}} \le 1 + \FNormS{\matX_{\cal S}^+ \matX_{\bar{\cal S}}}.$$
So, for $i=1,\dots,n$,
$$\sigma^{-2}_i(\matX_{\cal S}) \leq  \left(1+ \FNormS{\matX_{\cal S}^+  \matX_{\bar{\cal S}}  } \right) \cdot \sigma^{-2}_i(\matX)\,.
$$
We now bound $ \left(1+ \FNormS{\matX_{\cal S}^+  \matX_{\bar{\cal S}}  } \right) $.
Notice that $\matX_{\cal S}^+ \matX_{\bar{\cal S}}=\matY_{\cal S}^+ \matY_{\bar{\cal S}}$
and
$
\matY_{\cal S}^+ \matY \Pi =
    \left( \begin{array}{cc} \matY_{\cal S}^+\matY_{\cal S} & \matY_{\cal S}^+ \matY_{\bar{\cal S}} \end{array} \right)\,.
$
This implies that $\FNormS{\matY_{\cal S}^+ \matY \Pi} = \FNormS{\matY_{\cal S}^+\matY_{\cal S}} + \FNormS{\matY_{\cal S}^+ \matY_{\bar{\cal S}}}$.
$ \matY_{\cal S}^+\matY_{\cal S}$ is a projection;
so, $\FNormS{\matY_{\cal S}^+\matY_{\cal S}} = n$. We now have $\FNormS{\matY_{\cal S}^+ \matY \Pi } = n +  \FNormS{\matY_{\cal S}^+ \matY_{\bar{\cal S}}}$. $\matY \Pi$ has orthonormal rows; so,
$\FNormS{\matY_{\cal S}^+ \matY \Pi } = \FNormS{\matY^+_{\cal S}}$. So,
$\FNormS{\matY_{\cal S}^+ \matY_{\bar{\cal S}}} = \FNormS{\matY^+_{\cal S}} - n.$
Recall that,
$$
\FNormS{  \matY_{ \cal S}^+ } \le  \frac{ 4(m-n) + 1}{\left(k-n\right) \left( 1 + \frac{n-1}{m-n+1}\right) } \cdot n.
$$
Plugging that into the previous equality, we find that,
$$
\FNormS{\matY_{\cal S}^+ \matY_{\bar{\cal S}}} =  \frac{ 4(m-n) + 1}{\left(k-n\right) \left( 1 + \frac{n-1}{m-n+1}\right) } \cdot n - n =
\left(
\frac{ 4(m-n) + 1}{\left(k-n\right) \left( 1 + \frac{n-1}{m-n+1}\right) } -
\frac{\left(k-n\right) \left( 1 + \frac{n-1}{m-n+1}\right)}{\left(k-n\right) \left( 1 + \frac{n-1}{m-n+1}\right)} \right) \cdot n
\leq \frac{4m - 3n - k + 1}{ \left(k-n\right) \left( 1 + \frac{n-1}{m-n+1}\right) } \cdot n.
$$
This immediately gives a bound on $\left(1+ \FNormS{\matX_{\cal S}^+  \matX_{\bar{\cal S}}  } \right)$, which concludes the proof.

\paragraph{Running time.}
The running time of our algorithm is the sum of three terms, $T_{SVD} + T_{RRQR} + T_{Greedy}$,
where $T_{RRQR}$ and $T_{Greedy}$ correspond to the first and the second stage of our algorithm,
respectively, while $T_{SVD} = O(mn^2)$ is the time required to compute the right singular vectors of $\matX$.
Lemma 16 in~\cite{Bou11a} argues that the first stage of our algorithm can be implemented in $O(mn^2 \log m)$ time,
i.e. $T_{RRQR} = O(m n^2 \log m)$. A naive implementation of the second stage requires $O\left( mn^3 (k-n) \right)$ time. One
can also use the Sherman-Morisson formula and improve this to $O\left( n^3 + mn^2 (k-n) \right)$. Next, we argue that one
can use the fast SVD update algorithms from~\cite{GE94} and implement this step in $T_{Greedy} = O(mn(k-n))$. So, in total
our algorithm requires $O( mn^2 \log m + mnk )$, as advertised.

As with the proof in Theorem~\ref{thm1}, we start with some calculations, after which a description of a fast implementation of our algorithm
is immediate. Recall that we apply the greedy selection algorithm on $\matY$, which has orthonormal rows. Recall also that $\matY_{\cal S}$
constructed in the first stage of the algorithm. Let $\matY_{\cal S} = \matU \Sigma \matV\transp$ be an SVD of $\matY_{\cal S}$

Fix an index $i=n+1,n+2,...,m$; then,
\eqan{
\trace\left(  \left( \matX_{\cal S}\matX_{\cal S}\transp  - \x_i \x_i\transp  \right)^{-1}  \right) &\buildrel{(a)}\over{=}&
\trace\left(  \left( \matU\Sigma^2\matU\transp - \matU \Sigma \y_i \y_i\transp \Sigma \matU\transp  \right)^{-1}  \right) \\
&\buildrel{(b)}\over{=}&
\trace\left( \Sigma^{-2} + \frac{\Sigma^{-1} \y_i \y_i\transp
\Sigma^{-1}}{1 -  \y_i\transp \y_i }  \right) \\
&\buildrel{(c)}\over{=}&
\trace\left( \Sigma^{-2}\right) + \trace\left(\frac{\Sigma^{-1} \y_i \y_i\transp \Sigma^{-1}}{1 - \y_i\transp \y_i } \right)\\
&\buildrel{(d)}\over{=}&
\FNormS{\matX^{+}}  + \frac{1}{1-\TNormS{\y_i}} \cdot \trace\left( \Sigma^{-1} \y_i\transp \left( \Sigma^{-1} \y_i \right)\transp \right)   \\
&\buildrel{(e)}\over{=}&
\FNormS{\matX^{+}}  +  \cdot \frac{ \TNormS{ \Sigma^{-1} \y_i} }{1-\TNormS{\y_i}} \\
& \buildrel{(f)}\over{=} &
\FNormS{\matX^{+}} + \frac{ \sum_{j=1}^{n} \left( \y_{ij}^2 /\sigma_j^2 \right) } {1-\TNormS{\y_i}}
}

\end{proof} 

==> HC_LinearAlgebra.tex <==
\section{Linear Algebra}

\paragraph{Matrix norms.}
We use the Frobenius and the spectral norm of a matrix:
$ \FNorm{\matX} = \sqrt{\sum_{i,j} \matX_{ij}^2}$, and
$\TNorm{\matX} = \max_{\y:\TNorm{\y}=1}\TNorm{\matX \y}$, respectively.
For any two matrices $\matX$ and $\matY$ of appropriate dimensions, \math{\TNorm{\matX}\le\FNorm{\matX}\le\sqrt{\rank(\matX)}\TNorm{\matX}},
$\FNorm{\matX\matY} \leq \FNorm{\matX}\TNorm{\matY}$, and $ \FNorm{\matX\matY} \leq \TNorm{\matX} \FNorm{\matY}$. The latter two properties
are stronger versions of the standard submultiplicativity property:
$\XNorm{\matX\matY} \leq \XNorm{\matX}\XNorm{\matY}$. We will refer to these two stronger versions
as spectral submultiplicativity.
The notation $\XNorm{\matX}$ indicates that an expression holds for both $\xi = 2$ and $\xi = \mathrm{F}$.

\paragraph{Singular Value Decomposition.} \label{chap24}
The Singular Value Decomposition (SVD) of  $\matX \in \R^{n \times m}$ is:
%
\begin{eqnarray*}
\label{svdA} \matX
         = \underbrace{\left(\begin{array}{cc}
             \matU_{k} & \matU_{\rho-k}
          \end{array}
    \right)}_{\matU \in \R^{n \times \rho}}
    \underbrace{\left(\begin{array}{cc}
             \Sigma_{k} & \bf{0}\\
             \bf{0} & \Sigma_{\rho - k}
          \end{array}
    \right)}_{\Sigma \in \R^{\rho \times \rho}}
    \underbrace{\left(\begin{array}{c}
             \matV_{k}\transp\\
             \matV_{\rho-k}\transp
          \end{array}
    \right)}_{\matV\transp \in \R^{\rho \times m}},
\end{eqnarray*}
%
with singular values \math{\sigma_1\ge\ldots\sigma_k\geq\sigma_{k+1}\ge\ldots\ge\sigma_\rho > 0}.
Here, $\rho = \rank(\matX) $ and $k$ is some rank parameter $1 \le k \le \rho$.
We will often denote $\sigma_1$ as $\sigma_{\max}$ and $\sigma_{\rho}$ as $\sigma_{\min}$, and will use $\sigma_i\left(\matX\right)$ to denote the $i$-th singular value of $\matX$ when the matrix is not clear from the context. The matrices
$\matU_k \in \R^{n \times k}$ and $\matU_{\rho-k} \in \R^{n \times (\rho-k)}$ contain the left singular vectors of~$\matX$; and, similarly, the matrices $\matV_k \in \R^{m \times k}$ and $\matV_{\rho-k} \in \R^{m \times (\rho-k)}$ contain the right singular vectors of~$\matX$. It is well-known that $\matX_k=\matU_k \Sigma_k \matV_k\transp \in \R^{n \times m}$ minimizes \math{\XNorm{\matX - \matY}} over all
matrices \math{\matY \in \R^{n \times m}} of rank at most $k$. We use $\matA_{\rho-k} \in \R^{n \times m}$ to denote the matrix $\matA - \matA_k = \matU_{\rho-k}\Sigma_{\rho-k}\matV_{\rho-k}\transp \in \R^{n \times m}$. Also, $ \FNorm{\matX} = \sqrt{ \sum_{i=1}^\rho\sigma_i^2(\matX) }$ and $\TNorm{\matX} = \sigma_1(\matX)$. The best rank $k$ approximation to $\matX$ satisfies $\TNorm{\matX-\matX_k} = \sigma_{k+1}(\matX)$ and
$\FNorm{\matX-\matX_k} = \sqrt{\sum_{i=k+1}^{\rho}\sigma_{i}^2(\matX)}$.

\paragraph{Running time of SVD.}
Some of the algorithms of this paper require the computation of an SVD of a matrix and sometimes just updating it. Numerical algorithms for computing a SVD are always iterative: they proceed by improving approximations
to the true decomposition. The algorithm stops when the error has dropped below some low threshold $\epsilon$, which is usually close to the maximum accuracy attainable on the machine, e.g. $\epsilon = 10^{-16}$. The running time of these iterative algorithms depend on $\epsilon$ but it is hard to give an exact bound~\cite{Ste01}. In practice convergence is very fast, so this dependence is typically ignored in the analysis, which conveniently states that an SVD of an $n \times m$ matrix can be computed in $O\left( m n \min\{n,m\}\right)$ operations. We follow this paradigm and ignore terms related to accuracy in the runtime analysis, but only if the dependence is poly-log.

\paragraph{Eigenvalues and PSD matrices.}
Let $\matX \in \R^{n \times m}$ ($m \ge n$) and $\matA=\matX\transp \matX \in \R^{n \times n}$; then, for all $i=1, ...,n$, $\lambda_{i}\left(\matA\right) = \sigma_{i}^2\left(\matX\right)$ denotes the $i$-th eigenvalue of $\matA$. We will also use $\lambda_{\min}\left(\matA\right)$ and $\lambda_{\max}\left(\matA\right)$ to denote the smallest and largest eigenvalue of $\matA$, respectively.
Any matrix $\matA$ that can be written in this form  $\matA=\matX\transp \matX$ is called a Positive Semidefinite (PSD) matrix.
%; clearly, all eigenvalues of a PSD matrix are non-negative.

\paragraph{Moore-Penrose Pseudo-inverse.} Let $\matX \in \R^{n \times m}$ with SVD $\matX = \matU \Sigma \matV\transp$.
Then, $\matX^+ = \matV \Sigma^{-1} \matU\transp \in \R^{m \times n}$
denotes the Moore-Penrose pseudo-inverse of $\matX$ ($\Sigma^{-1}$ is the inverse of $\Sigma$),
i.e. the unique $m \times n$ matrix satisfying all four properties:
$\matX = \matX \matX^+ \matX$,
$\matX^+ \matX \matX^+ = \matX^+$,
$(\matX \matX^+ )\transp = \matX \matX^+$, and
$(\matX^+ \matX )\transp = \matX^+\matX$.
By the SVD of $\matX$ and $\matX^+$, it is easy to verify
that, for all $i=1,...,\rho = \rank(\matX) = \rank(\matX^+)$,
$\sigma_i(\matX^+) = 1 / \sigma_{\rho - i + 1}(\matX)$.
We will also use the following standard result.
\begin{lemma}
\label{lem:pseudo} Let $\matA \in \R^{m \times n}, \matB \in \R^{n \times \ell}$; then,
\math{(\matA\matB)^+=\matB^+\matA^+} if at least one
of the three is true:
(\rn{1}) \math{\matA\transp\matA=\matI_n};
(\rn{2}) \math{\matB\transp\matB=\matI_{\ell}};
or, (\rn{3}) $\rank(\matA) = \rank(\matB) = n$.
\end{lemma}

\paragraph{Trace.} The trace of a square matrix $\matA$, denoted as $\trace\left( \matA \right)$ equals the sum of the diagonal elements of $\matA$,
which is exactly the same to the sum of the eigenvalues of $\matA$. Using this definition, it follows that, for any matrix $\matX$ we have
$\trace\left( \matX\transp \matX \right) = \FNormS{\matX}$. Another useful property, which connects the trace operator with the pseudo-inverse, is the
following. Let $\matX \in \R^{n \times m}$ with $m > n$ and $\rank(\matX)=n$.
Then, $\FNormS{\matX^+} = \trace\left( \left( \matX\matX\transp \right)^{-1} \right)$.

\paragraph{Sherman-Morrison formula.} Let $\matA$ be a square full rank matrix of dimension $n$. Let $\x$ is an $n$-vector.
The Sherman-Morrison formula (see, for example, Section 2.1.3 in~\cite{GV89}) describes a convenient way to compute the inverse of
$\matA + \x \x\transp$ (a rank one update to $\matA$) with respect to the inverse of $\matA$:$$ \left( \matA + \x \x\transp \right)^{-1} = \matA^{-1} - \frac{\matA^{-1} \x \x\transp \matA^{-1}}{ 1 + \x\transp \matA^{-1} \x }. $$
Notice that given $\matA^{-1}$ and $\x$ one can compute $\left( \matA + \x \x\transp \right)^{-1}$ in
$O\left(n^2 \right)$ operations.

\paragraph{Determinant and Cramer's rule.}
Let $\matA \in \R^{n \times n}$ be a square matrix of arbitrary size.
We denote the determinant of $\matA$ by $\det(\matA)$.
We recall a few properties related to the determinant.
For any matrix $\matA$ we have $\det(\matA\transp)=\det(\matA)$,
and for any two matrices $\matA$ and $\matB$ of the same dimension we have
$\det(\matA \matB) = \det(\matA) \det(\matB)$.
For any square matrix $\matA$ the determinant is equal to the product
of the eigenvalues of the matrix. A square matrix $\matA$ is singular if and only if $\det(\matA)=0$.

For a matrix $\matA$, an index $i$ and a vector $\v$, we denote by
$\matA(i \rightarrow \v)$ the matrix obtained after replacing the
$i$-th column of $\matA$ by $\v$. Notice that for $\matA$ and $\matB$ of
the same dimension we have $\det(\matA) \det(\matB(i \rightarrow \v)) = \det( (\matA \matB)(i \rightarrow \matA \v) )$.
Finally, recall Cramer's rule, which gives a formula for computing the components of
$\x=\matA^{-1}\b$ in terms of determinants. In our notation, the rule states
that $\x_{i}$, the $i$-th position in $\x$, can be computed using the formula,
$$\x_{i}=\frac{\det(\matA(i \rightarrow \b))}{\det(\matA)}\,.$$

\paragraph{Adjugate Matrix.} Let $\matA$ is a square matrix of dimension $n$.
The adjugate of $\matA$, denoted as $\Adj\left( \matA \right)$, is a square
matrix of dimension $n$ defined as follows. Let $\matX$ is a square matrix
of dimension $n$, where for $i=1,\dots,n$ and $j=1,\dots,n$, $\matX_{ij} = (-1)^{(i+j)}\det( \matA_{ij})$,
where $\matA_{ij}$ is the matrix that results from deleting row $i$ and column $j$ of $\matA$.
Then, $\Adj\left( \matA \right) = \matX\transp$.
The adjugate matrix connects the determinant of a non-singular matrix with its inverse.
Let $\matA$ is a square invertible matrix; then, $\matA^{-1} = \det\left( \matA \right)^{-1} \cdot  \Adj\left( \matA \right)$.


\paragraph{Volume Sampling.} Let $\matX$ be a full rank matrix with arbitrary dimensions $n \times m$.
Let $\cal S$ $\subseteq [m]$ has cardinality $k$ for $1 \le k \le m$. Let, $i=1,2,\dots\ell=\binom{m}{k}$.
For all possible subsets of cardinality $k$, define probabilities,
$$ p_i = \frac{ \det\left( \matX_{{\cal S}_i} \matX_{{\cal S}_i}\transp \right) }{ \sum_{j=1}^{\ell} \det\left( \matX_{{\cal S}_j} \matX_{{\cal S}_j}\transp \right) }. $$
We will denote with $S_{k}(\matX)$ the above distribution of $k$-subsets in the matrix $\matX$. For example,
${\cal S} \sim S_{k}(\matX)$ denotes the fact that $\cal S$ is the outcome of a random experiment using
the above distribution. Notice that if $\matA$ is a square non-singular matrix then
$S_{k}(\matA \matX) = S_{k}(\matX)$ (this follows from the fact that $\det((\matA \matX)_{\cal S}(\matA \matX)\transp_{\cal S}) = \det(\matA)^2 \det(\matX_{\cal S}\matX\transp_{\cal S})$ for every $\cal S$).

An efficient algorithm for sampling a set from $S_{n}(\matX)$ was first suggested by Deshpande and Rademacher~\cite{DR10}. This algorithm was recently improved by Guruswami and Sinop, who showed how
to sample such a subset in $O(n^{3}m)$ time~\cite{GK11}.
There is currently no algorithm for sampling from $S_{k}(\matX)$ for an arbitrary $k \geq n$.

\begin{lemma}[Cauchy-Binet formula] Let $\matA \in \R^{n \times m}, \matB \in \R^{n \times m}$, and $m\ge n$. Then,
$ \det(\matA \matB\transp) = \sum_{{\cal S} \in \binom{[m]}{n}} \det(\matA_{\cal S}) \det( (\matB\transp)_{\cal S})\,.$
\end{lemma}
\begin{lemma}[Lemma 6 in~\cite{GK11}]
\label{GK11-lem6}
Let $\lambda_1 \ge \lambda_2 \ge ... \ge \lambda_m,$ denote the eigenvalues of $\matA \in \R^{m \times m}$.
Let $1 \le k \le m$.
Then,
$ \sum_{{\cal S} \in \binom{[m]}{k}} \det\left( \matA_{{\cal S},{\cal S}} \right) = \sum_{{\cal S} \in \binom{[m]}{k}} \prod_{i \in {\cal S}} \lambda_i.$
Here, $\matA_{{\cal S},{\cal S}} \in \R^{k \times k}$ denotes the submatrix of $\matA$ corresponding to the rows and the columns in ${\cal S}$
$\subseteq [m]$, which has cardinality $k$.
\end{lemma}


==> HC_Main_Hard.tex <==

%\section{Main Results}

%\subsection{Hardness of Approximation}\label{sec:opt1}
%\begin{theorem}\label{thm:hard}
%The Frobenius norm version of the subset selection problem of Definition~\ref{def:prob} is NP-hard. 
%\end{theorem}
%\begin{proof}
%We should give it a try...
%\end{proof}


==> HC_ProofHoog.tex <==
\section{Proof of Correctness of Greedy Removal}
We first prove that the bound holds for $k = m - 1$.
Let ${\cal T} \sim S_{m-1}(\matX)$. Lemma~\ref{lem:volrand} implies that
$$\Expect{\FNormS{\matX_{\cal T}^{+}}}\leq\frac{m-n+1}{m-n} \cdot \FNormS{\matX^{+}}\,.$$
So, there exists $\hat{\cal S} \subseteq [m]$ of cardinality $m-1$ such that
$$
\FNormS{\matX^+_{\hat{\cal S}}}\leq \frac{m - n + 1}{m - n} \cdot \FNormS{\matX^+}\,.
$$
Notice that $\hat{\cal S}$ must have a non-zero probability of sampling (it is a discrete distribution).
Therefore, $\det(\matX_{\hat{\cal S}}\matX\transp_{\hat{\cal S}})\neq 0$, which  implies that $\matX_{\hat{\cal S}}$ is full rank.
Also, notice that greedy removal finds a subset $\tilde{\cal S} \subseteq [m]$ of cardinality $m-1$ and $\rank(\matX_{\tilde{\cal S}})=n$
which is at least as good as $\hat{\cal S}$,
$$ \FNormS{\matX^+_{\tilde{\cal S}}} \le \FNormS{\matX^+_{\hat{\cal S}}}\leq \frac{m - n + 1}{m - n} \cdot \FNormS{\matX^+}.$$
So, the bound holds for $k=m-1$. The bound for $\cal S$ of cardinality $k$ now follows by induction. 

==> HC_TitleAbstract.tex <==
\title{\bf Faster Subset Selection for Matrices and Applications}

\author{
{\bf Haim Avron} \\
Business Analytics \& Mathematical Sciences \\
IBM T.J. Watson Research Center \\
haimav@us.ibm.com
\and
{\bf Christos Boutsidis} \\
Business Analytics \& Mathematical Sciences \\
IBM T.J. Watson Research Center \\
cboutsi@us.ibm.com
}

\maketitle

\begin{abstract}
We study the following problem of \emph{subset selection} for matrices:
given a matrix $\matX \in \R^{n \times m}$ ($m > n$) and a sampling
parameter $k$ ($n \le k \le m$), select a subset of $k$ columns from
$\matX$ such that the pseudo-inverse of the sampled matrix has as
smallest norm as possible. In this work, we focus on the Frobenius and
the spectral matrix norms.
We describe several novel (deterministic and randomized) approximation algorithms for this
problem with approximation bounds that are optimal up to constant factors.
Additionally, we show that the combinatorial problem of finding a low-stretch spanning tree in an undirected graph
corresponds to subset selection, and discuss various implications of this reduction.
\end{abstract}

